The Geometry of Neural Nets' Parameter Spaces Under Reparametrization

Model reparametrization, which follows the change-of-variable rule of calculus, is a popular way to improve the training of neural nets. But it can also be problematic since it can induce inconsistencies in, e.g., Hessian-based flatness measures, optimization trajectories, and modes of probability densities. This complicates downstream analyses: e.g. one cannot definitively relate flatness with generalization since arbitrary reparametrization changes their relationship. In this work, we study the invariance of neural nets under reparametrization from the perspective of Riemannian geometry. From this point of view, invariance is an inherent property of any neural net if one explicitly represents the metric and uses the correct associated transformation rules. This is important since although the metric is always present, it is often implicitly assumed as identity, and thus dropped from the notation, then lost under reparametrization. We discuss implications for measuring the flatness of minima, optimization, and for probability-density maximization. Finally, we explore some interesting directions where invariance is useful.

==> contents/91_background.tex <==
%!TEX root = ../main.tex

\section{Background: Riemannian Geometry}
\label{app:background}

\begin{figure*}[t]
  \centering

  \includegraphics[width=0.75\linewidth, height=0.215\textheight]{figs/manifold}

  \caption{A pictorial summary of this section. Note that all quantities are defined at \(p\). Faint grids on the manifold represents coordinates---imagine having an \(\R^2\) mesh wrapped around \(M\).}

  \label{fig:manifold}
\end{figure*}

\subsection{Smooth Manifolds and Coordinates}

A \defword{manifold} of dimension \(n\) is a topological space that is locally homeomorphic to \(\R^n\). For practical tractability, throughout this document that an \(n\)-manifold is \emph{globally} homeomorphic to \(\R^n\).

\begin{assumption}
  The manifold considered here can always be covered by a global coordinate chart. \qedex
\end{assumption}

Let \(M\) be such a manifold. A \defword{coordinate system} on \(M\) is a homeomorphism \(\theta: M \to \R^n\), representing an abstract point \(p\) of \(M\) with an \(n\)-tuple of real numbers, \(\theta(p) := (\theta^1(p), \dots, \theta^n(p))\). In this case, \(p\) and \(\theta(p)\) can interchangeably be used to refers to a point in \(M\).

We can also call a coordinate system of \(M\) as a \defword{parametrization} since if \(f \in C^\infty(M)\), then different coordinate representations of \(M\) can be seen as different parametrizations of \(f\).

\begin{example}
  Let \(M := \{ p_x := \N(x \mid \mu, \sigma^2) : \mu \in \R, \sigma^2 \in \R_{> 0} \}\). Then, we can use the following coordinates:
  %
  \begin{itemize}
    \item \(\theta(p_x) := (\mu, \sigma^2) \in \R \times \R_{> 0}\), or
    %
    \item \(\theta(p_x) := (\mu, \log \sigma^2) \in \R \times \R\).
  \end{itemize}
  %
  In any case, \(M\) is of dimension 2 because the codomain of \(\theta\) is isomorphic to \(\R^2\). \qedex
\end{example}

A coordinate system is an additional structure on top of a manifold, and we are free to choose it. It is simply a way of representing abstract points (and other abstract objects) in \(M\) with more concrete objects. It follows that abstract objects of \(M\) must \emph{not} dependant on the choice of coordinates, otherwise we would have inconsistencies. In other words, abstract objects of \(M\) are coordinate-independent and thus \emph{invariant} to the choice of coordinates.

\begin{example}
  Let us use a real-world example. Let us consider an object \(p\) which consists of paper pages bundled together and a cover. Everybody knows what this object is. But it is still quite abstract and so different cultures assigns different words to it. In English, it is represented by the word ``book''; in German ``Buch'', etc.

  Here, the manifold consists of all objects on earth, and we have considered two coordinate systems for representing points in the manifold: English and German languages. The word ``book'', ``Buch'' are the coordinate representation \(\theta(p)\) of the object \(p\) in the English and German coordinates, respectively. Note that \(p\) is invariant to the choice of words for representing it---\(\theta(p)\) refers to the same object, regardless of the language system \(\theta\). \qedex
\end{example}


\subsection{Tangent Vectors}

Let \(p \in M\). We define a \defword{tangent space to \(\mM\) at \(p\)}, denoted by \(T_p M\), to be the set \(\{ (p, v) : v \in \R^n \}\). A \defword{tangent vector at \(\vp\)} is an element of \(T_p M\). We can think of \(v\) as an ``arrow'' and \(p\) as the ``root'' of the arrow. One can show that \(T_p M\) is an \(n\)-dimensional real vector space and thus isomorphic to \(\R^n\) and to the coordinate representation of \(M\).

A tangent vector \(v \in T_p M\) provides a way of taking directional derivatives of smooth functions on \(M\). This is because \(v\) yields a map \(D_v \vert_p : C^\infty(M) \to \R\) by
%
\[
  D_v \vert_p (f) := \left. \frac{d}{dt} \right\vert_{t=0} f(\theta(p) + tv).
\]
%
That is, \(v\) takes the directional derivative of \(f\) in the direction \(v\) at \(p\). We can think of \(v\) and \(D_v \vert_p\) interchangeably as an element of \(T_p M\), because the map \(v \mapsto D_v \vert_p\) is an isomorphism---we can write
%
\begin{equation} \label{eq:derivation}
  v(f) = D_v \vert_p (f) .
\end{equation}
%

Let \((e_i \vert_p)_{i=1}^n\) be the standard basis for \(T_pM \simeq \R^n\). Then, we can write \(v = \sum_{i=1} v^i e_i \vert_p\) for some real numbers \((v^i)\), and \(D_v \vert_p (f)\) can be written more concretely via the chain rule by
%
\[
  D_v \vert_p(f) = \sum_{i=1}^n v^i \frac{\partial f}{\partial \theta^i}(p) ,
\]
%
i.e., it is just a dot product between the components of \((v^i)\) of \(v\) and the \(n\)-tuple of partial derivatives of \(f\) at \(p\). In particular, note that,
%
\begin{equation} \label{eq:coordinate_basis}
  D_{e_i} \vert_p = \left. \frac{\partial}{\partial \theta^i} \right\vert_p .
\end{equation}
%
From here and the fact that \(v \in T_pM\) is represented by \(D_v \vert_p\), it is therefore clear that the \(n\) partial derivatives
%
\[
  \left. \frac{\partial}{\partial \theta^1} \right\vert_p, \dots, \left. \frac{\partial}{\partial \theta^n} \right\vert_p \qquad \text{defined by} \qquad \left(\left. \frac{\partial}{\partial \theta^i} \right\vert_p \right) (f) = D_{e_i} \vert_p (f) = \frac{\partial f}{\partial \theta^i}(p)
\]
%
form a basis for \(T_p M\). The vectors \(\partial/\partial \theta^i \vert_p\) are called the \defword{coordinate basis vectors at \(\vp\)} associated with the given coordinate system \(\theta\). So, any tangent vector \(v \in T_pM\) can be written uniquely as a linear combination
%
\[
  v = \sum_{i=1}^n v^i \left.\frac{\partial}{\partial \theta^i}\right\vert_p .
\]
%
In other words, under a choice of coordinates \(\theta\), the vector \(v\), just like the point \(p \in M\), is also represented by an \(n\)-tuple of real numbers \((v^i)\).


\subsection{Change of Coordinates}

Let \(\varphi: M \to M\) be a diffeomorphism (a smooth map that has a smooth inverse). We call \(\varphi\) a \defword{change of coordinates of \(\mM\)} or \defword{reparametrization of \(\mM\)}. For each \(p \in M\) we define
%
\[
  d\varphi_p : T_pM \to T_{\varphi(p)} M ,
\]
%
called the \defword{differential of \(\boldsymbol{\varphi}\) at \(\vp\)}, as follows. Given \(v \in T_pM\), we let \(d\varphi_p(v)\) be the tangent vector at \(\varphi(p)\) that acts on a function \(f \in C^\infty(M)\) by
%
\[
  d\varphi_p(v)(f) := D_v \vert_{F(p)} (f \circ \varphi) .
\]
%
One can show that \(d\varphi_p\) is linear, and it is an isomorphism between \(T_p M\) and \(T_{\varphi(M)}\) and \((d\varphi_p)^\inv = d(\varphi^\inv)_{\varphi(p)}\).


Let \((\theta^i)\) and \((\wt{\theta}^i)\) be two coordinate systems assigned to the domain and codomain of \(\varphi\), respectively. We would like to know the coordinate representation of the differential \(d\varphi_p\). The components of the matrix of \(d\varphi_p\) is given by its action on a basis vector as follows (via the chain rule):
%
\begin{align*}
  d\varphi_p\left(\left.\frac{\partial}{\partial \theta^i}\right\vert_p\right)(f) = \left(\left. \frac{\partial}{\partial \theta^i} \right\vert_p \right) (f \circ \varphi) = \sum_{j=1}^n \frac{\partial f}{\partial \wt{\theta}^j}(\varphi(p)) \frac{\partial \varphi^j}{\partial \theta^i}(p) = \left( \sum_{j=1}^n \frac{\partial \varphi^j}{\partial \theta^i}(p) \left.\frac{\partial}{\partial \wt{\theta}^j}\right\vert_{\varphi(p)} \right) (f) .
\end{align*}
%
Therefore,
%
\begin{equation} \label{eq:differential_action}
  d\varphi_p\left(\left.\frac{\partial}{\partial \theta^i}\right\vert_p\right) = \sum_{j=1}^n \frac{\partial \varphi^j}{\partial \theta^i}(p) \left.\frac{\partial}{\partial \wt{\theta}^j}\right\vert_{\varphi(p)} .
\end{equation}
%
In other words, the matrix of \(d\varphi_p\) in terms of the coordinate basis induced by the choice of coordinates \(\theta\) on \(M\) is given by the \(n \times n\) array
%
\[
  \mJ(p) := \begin{pmatrix}
    \frac{\partial \varphi^1}{\partial \theta^1}(p) & \dots & \frac{\partial \varphi^1}{\partial \theta^n}(p) \\
    %
    \vdots & \ddots & \vdots \\
    %
    \frac{\partial \varphi^n}{\partial \theta^1}(p) & \dots & \frac{\partial \varphi^n}{\partial \theta^n}(p)
  \end{pmatrix} .
\]
%
This is none other than the Jacobian matrix of \(\varphi\) at \(p\).

Therefore, by \eqref{eq:differential_action}, if we have \(v = \sum_{i=1}^n v^i \left.\frac{\partial}{\partial \theta^i}\right\vert_p \in T_pM\), then under a change of coordinates \(\varphi(p)\), by linearity, the vector \(v\) becomes
%
\begin{equation} \label{eq:vector_transform}
  \begin{aligned}
    d\varphi_p(v) &= d\varphi_p\left(\sum_{i=1}^n v^i \left.\frac{\partial}{\partial \theta^i}\right\vert_p\right) = \sum_{i=1}^n v^i d\varphi_p\left(\left.\frac{\partial}{\partial \theta^i}\right\vert_p\right) = \sum_{i=1}^n v^i \sum_{j=1}^n \frac{\partial \varphi^j}{\partial \theta^i}(p) \left.\frac{\partial}{\partial \wt{\theta}^j}\right\vert_{\varphi(p)} \\
      %
      &= \sum_{j=1}^n \left(\sum_{i=1}^n v^i \frac{\partial \varphi^j}{\partial \theta^i}(p)\right) \left.\frac{\partial}{\partial \wt{\theta}^j}\right\vert_{\varphi(p)} \in T_{\varphi(p)}M .
  \end{aligned}
\end{equation}
%
In other words, the ``new'' components \(\wt{\vv} := (\wt{v}^1, \dots, \wt{v}^n)\) of \(\wt{v} := d_{\varphi_p}(v) \in T_{\varphi(p)}M\) is given in terms of the ``old'' components \(\vv := (v^1, \dots, v^n)\) by \(\wt{\vv} = \mJ(p) \vv\), i.e. it is multiplied by the Jacobian of the change of coordinates \(\varphi\) at \(p\).

Correspondingly, the ``old'' components \(\vv\) is obtained via the ``new'' ones by \(\vv = \mJ^\inv(p) \wt{\vv}\). I.e. \emph{``to get the old ones, multiply the new ones by the inverse Jacobian''}.


\subsection{Tangent Covectors}

Let \(M\) be an \(n\)-manifold with coordinates \(\theta\) and let \(p \in M\). We define a \defword{(tangent) covector on \(\mT_{\vp} \mM\)} to be a real-valued linear functional \(\omega: T_pM \to \R\) on \(T_pM\). The space of all tangent covectors on \(T_pM\) is called the \defword{cotangent space of \(\mT_{\vp} \mM\)}, denoted by \(T^*_pM\)---it is a dual space of the vector space \(T_pM\).

Given any basis \((e_i)\) on \(T_pM\), the covectors \(\epsilon^1, \dots, \epsilon^n \in T^*_pM\) defined by
%
\[
  \epsilon^i(e_i) = \delta^i_j ,
\]
%
where \(\delta^i_j\) is the Kronecker delta, forms a basis for \(T^*_pM\), and so \(\dim T^*_p M = \dim T_p M = n\). In particular, given a coordinate basis \((\partial/\partial \theta^i \vert_p)\), we obtain a basis, say, \((\lambda^i \vert_p)\) for \(T^*_p M\). I.e. a covector \(\omega \in T^*_p M\) can be uniquely written as \(\omega = \sum_{i=1}^n \omega_i \lambda^i \vert_p\) for some real numbers \((\omega_i, \dots, \omega_n)\)---given a coordinate system, covectors can also be represented by an array of real numbers of length \(n\).

Based on the definition, we can then see how the component \(\omega_i\) of \(\omega\) is obtain, by applying it to the coordinate basis vector \(\partial/\partial \theta^i \vert_p\):
%
\begin{equation} \label{eq:covector_component}
  \omega\left( \left.\frac{\partial}{\partial \theta^i}\right\vert_p \right) = \sum_{j=1}^n \omega_j \lambda^j\left( \left.\frac{\partial}{\partial \theta^i}\right\vert_p \right) = \sum_{j=1}^n \omega_j \delta^j_i = \omega_i .
\end{equation}
%
It also follows that the action of \(\omega\) on \(v \in T_pM\) is
%
\begin{equation} \label{eq:covector_action}
  \omega(v) = \sum_{i=1}^n \omega_i v^i ,
\end{equation}
%
i.e. it is just the dot product of the component arrays of \(\omega\) and \(v\).

Suppose \(\wt{\theta}\) is another coordinate system of \(M\). At \(p\), it induces a dual basis \((\wt{\lambda}^i \vert_p)\). Recall that a vector \(v\) is represented by \(\wt{v}\) from \eqref{eq:vector_transform} in this new coordinates. We would like to know the components \((\wt{\omega}^i)\) of \(\omega\) in this new coordinates. First, notice that \(\wt{\omega}(\wt{v}) = \omega(v)\) since both vectors and covectors are coordinate-invariant objects of \(M\). Then,
%
\begin{equation*}
  \wt{\omega}(\wt{v}) = \sum_{i=1}^n \wt{\omega}_i \left(\sum_{j=1}^n v^j \frac{\partial \varphi^i}{\partial \theta^j}(p)\right) = \sum_{j=1}^n \left( \sum_{i=1}^n \wt{\omega}_i \frac{\partial \varphi^i}{\partial \theta^j}(p) \right) v^j \stackrel{\text{def}}{=} \omega(v) .
\end{equation*}
%
So, from \eqref{eq:covector_action}, we can identify the component \(\omega_i\) of \(\omega\) under the ``old'' coordinates from the component \(\wt{\omega}_i\) under the ``new'' coordinates by
%
\[
  \omega_i = \sum_{i=1}^n \wt{\omega}_i \frac{\partial \varphi^i}{\partial \theta^j}(p) .
\]
%
In matrix notation, this is \(\vomg = \mJ(p) \wt{\vomg}\). Thus, the components of covectors transform \emph{the opposite way} compared to the components of vectors. We call the transformation of vectors \defword{contravariant transformation}, while that of covectors \defword{covariant transformation}. For this reason, we also call tangent vectors and covectors as \defword{contravariant vectors} and \defword{covariant vectors}, respectively.


\subsection{The Differential of a Function}

Let \(M\) be an \(n\)-manifold with coordinates \(\theta\), \(p \in M\), and let \(f \in C^\infty(M)\). We define a covector \(df\), called the \defword{differential of \(\vf\)}, by its action on a tangent vector \(v \in T_pM\) at \(p\):
%
\[
  df_p(v) := v(f) .
\]

Let us now find out the coordinate representation of this covector. Let \(\partial/\partial \theta^i \vert_p\) and \(\lambda^i \vert_p\) be the tangent and dual bases induced by \(\theta\), respectively. Since \(df_p\) is a covector, it can be written as \(df_p = \sum_{i=1}^n \omega_i(p) \lambda^i \vert_p\) for some functions \(\omega_i: M \to \R\). Then, by \eqref{eq:covector_component}, \eqref{eq:coordinate_basis}, and the definition of \(df_p\):
%
\[
  \omega_i(p) = df_p\left( \left.\frac{\partial}{\partial \theta^i}\right\vert_p \right) = D_{e_i} \vert_p (f) = \frac{\partial f}{\partial \theta^i}(p) .
\]
%
So, we have
%
\[
  df_p = \sum_{i=1}^n \frac{\partial f}{\partial x^i}(p) \lambda^i \vert_p ,
\]
%
and thus, the coordinate representation of \(df_p\) is the \(n\)-array \(\vd(p) := (\partial f/\partial \theta^1(p), \dots, \partial f/\partial \theta^n(p))\). So, the gradient ``vector'' \(\nabla f (p)\) we all know from Calculus is actually a covector! This is the reason why standard gradient descent is not invariant w.r.t. change of coordinates, even though \(df_p\) is: the ``gradient'' used as a descent direction is actually a covector, but a gradient is actually a vector, thus, it uses the wrong transformation rule under a reparametrization! To make it invariant, we have to first translate \(df_p\) to a ``real'' gradient. This is done via a Riemannian metric, which we shall discuss next.


\subsection{Riemannian Metrics}

Let \(M\) be an \(n\)-manifold. A \defword{Riemannian metric} on \(M\) is a smooth covariant 2-tensor field \(g\) whose value \(g_p\) at \(p \in M\) is an inner product on \(T_pM\). That is, at each \(p\), the bilinear map \(g_p: T_pM \times T_pM \to \R\) takes two tangent vectors \(u, v \in T_pM\) and outputs a real number s.t. \(g_p(u, v) = g_p(v, u)\), and \(g_p(v, v) \geq 0\) where \(g_p(v, v) = 0\) if and only if \(v = 0\). The pair \((M, g)\) is called a \defword{Riemannian manifold}. As a side note, a common notation is \(g_p(u, v) = \inner{u, v}\).

Suppose \(\theta\) is a coordinate system on \(M\). A Riemannian metric \(g\) can then be represented by \(n^2\) smooth functions \(g_{ij}: M \to \R\), characterized by the coordinate basis \((\partial/\partial \theta^i)\):
%
\[
  g_{ij}(p) = \inner{\partial/\partial \theta^i \vert_p, \partial/\partial^j \vert_p} \qquad \text{for all } p \in M .
\]
%
Moreover, it is represented by an \(n \times n\) matrix \(\mG(p)\) whose components are
%
\[
  \mG(p) = \begin{pmatrix}
    g_{11}(p) & \dots & g_{1n}(p) \\
    \vdots & \ddots & \vdots \\
    g_{n1}(p) & \dots & g_{1n}
  \end{pmatrix} .
\]
%
Thus, if \(u, v \in T_pM\) with representations \(\vu, \vv\), respectively, then \(\inner{u, v} = \vu^\top \mG(p) \vv\).

Under a change of coordinates \(\varphi\), the representation \(\mG(p)\) of \(g\) at \(p\) transforms as follows. First, recall that to obtain the ``new'' representations \(\wt{\vu}, \wt{\vv}\) of the tangent vectors  \(\vu, \vv\), we multiply the latter with the Jacobian \(\mJ^\inv(p)\) of \(\varphi\). Since \(g\) is also an invariant object on \(M\), we expect that \(\vu^\top \mG(p) \vv = \wt{\vu}^\top \wt{\mG}(\varphi(p)) \wt{\vv}\). So, the matrix of the ``old'' metric from the ``new'' one is obtained via
%
\[
  \wt{\vu}^\top \wt{\mG}(\varphi(p)) \wt{\vv} = (\mJ(p) \vu)^\top \wt{\mG}(\varphi(p)) (\mJ(p) \vv) = \vu^\top \mJ(p)^\top \wt{\mG}(\varphi(p)) \mJ(p) \vv \stackrel{\text{def}}{=} \vu^\top \mG(p) \vv .
\]
%
Therefore, we can identify \(\mG(p)\) with \(\mJ(p)^\top \wt{\mG}(\varphi(p)) \mJ(p)\). This metric is also called the \defword{pullback metric of \(\wt{\vg}\) by \(\boldsymbol{\varphi\)}} and denoted by \(\varphi^*\wt{g}\). This is because we ``pull the new representation of the metric back to the old representation''.

\begin{example}[The Euclidean Metric]
  The \defword{Euclidean metric} is the Riemannian metric \(\overbar{g}\) on \(\R^n\) whose value at each \(x \in \R^n\) is the usual dot product on \(T_x \R^n\) under the natural identification \(T_x\R^n \simeq \R^n\).
  This means that for \(v, w \in T_x \R^n\) written in standard (Cartesian) coordinates \((x^1, \dots, x^n)\) as \(v = \sum_i v^i \partial/\partial x^i \vert_x\), \(w = \sum_i w^i \partial/\partial x^i \vert_x\), we have
  %
  \begin{equation*}
      \inner{v, w}_{\overbar{g}} = \delta_{ij} v^i w^i = \sum_{i=1}^n v^i w^i .
  \end{equation*}
  %
  Let \((M,g)\) be a Riemmanian manifold. The metric \(g\) is said to be \defword{flat} if there is a local isometry from \((M,g)\) to \((\R^n, \overbar{g})\).
  \qedex
\end{example}

\begin{theorem} \label{thm:flatness_criterion}
  Let \((M,g)\) be a Riemannian manifold. The following are equivalent:
  %
  \vspace{-0.5em}
  \begin{enumerate}[(a), itemsep=0.1em,topsep=0.1em,parsep=0pt,partopsep=0pt]
      \item \(g\) is flat.
      %
      \item For each \(p \in M\) there exists a smooth coordinate chart which domain contains \(p\), in which \(g\) has the coordinate representation \(g_{ij} = \delta_{ij}\).
      %
      \item For each \(p \in M\) there exists a smooth coordinate chart which domain contains \(p\), in which every coordinate basis is orthonormal. \qed
  \end{enumerate}
\end{theorem}

\Cref{thm:flatness_criterion} tells us that we can only find a coordinate chart s.t. \(g\) is represented by the identity matrix when the manifold is flat.
In this case, one needs to find an orthonormal coordinates. For the Euclidean space, this coordinates is simply the standard Cartesian coordinates.
Note that the Cartesian coordinate system is the default coordinates used in applications.


\subsection{Tangent-Cotangent Isomorphism}

In important property of Riemannian metrics is that they allow us to convert vectors to covectors and vice-versa. Given a metric \(g\) on \(M\), at each \(p \in M\) we define a map \(\wh{g}_p: T_pM \to T^*_pM\) by the action of the resulting covector:
%
\[
  \underbrace{(\wh{g}_p(u))}_{\in T^*_pM}(v) = g_p(u, v) = \inner{u, v} ,
\]
%
for all \(u, v \in T_pM\). In other words, \(\wh{g}_p(u) = \inner{u, \cdot}\) Using the coordinate representations \(\mG(p), \vu, \vv\) of \(g_p\), \(u\), \(v\), we can write
%
\[
  \wh{g}_p(u) = \mG(p) \vu .
\]
%
That is, to convert a vector \(u\) into a covector, we multiply it with the metric.

The map \(\wh{g}_p\) is actually an isomorphism because \(\mG\) is invertible, so we have also \(\wh{g}^\inv_p: T^*_pM \to T_pM\) via
%
\[
  \wh{g}^\inv_p(\omega) = \mG^\inv(p) \vomg .
\]
%
for any \(\omega \in T^*_pM\). Hence, to get a vector from a covector, we multiply the latter by the \emph{inverse} metric.

Recalling that in elementary Calculus the gradient is a vector (field), while so far we only have the differential which is a covector (field), we can use this isomorphism to finally obtain the former. Let \(p \in M\) and \(f \in C^\infty(M)\). We define the \defword{gradient of \(\vf\) at \(\vp\)} by
%
\[
  \grad f_p := \wh{g}^\inv_p(df_p) .
\]
%
In other words, the coordinate representation \(\vg(p)\) of \(\grad f_p\) is given by \(\vg(p) = \mG^\inv(p) \vd(p)\).


==> contents/93_add_experiments.tex <==
\section{The Hessian's trace under reparameterization}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

